Bidirectional Language Models Are Also Few-shot Learners

Large language models such as GPT-3 (Brown et al., 2020) can perform arbitrary tasks without undergoing fine-tuning after being prompted with only a few labeled examples. An arbitrary task can be reformulated as a natural language prompt, and a language model can be asked to generate the completion, indirectly performing the task in a paradigm known as prompt-based learning. To date, emergent prompt-based learning capabilities have mainly been demonstrated for unidirectional language models. However, bidirectional language models pre-trained on denoising objectives such as masked language modeling produce stronger learned representations for transfer learning. This motivates the possibility of prompting bidirectional models, but their pre-training objectives have made them largely incompatible with the existing prompting paradigm. We present SAP (Sequential Autoregressive Prompting), a technique that enables the prompting of bidirectional models. Utilizing the machine translation task as a case study, we prompt the bidirectional mT5 model (Xue et al., 2021) with SAP and demonstrate its few-shot and zero-shot translations outperform the few-shot translations of unidirectional models like GPT-3 and XGLM (Lin et al., 2021), despite mT5's approximately 50% fewer parameters. We further show SAP is effective on question answering and summarization. For the first time, our results demonstrate prompt-based learning is an emergent property of a broader class of language models, rather than only unidirectional models.

==> Bidirectional Camera-Ready/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Bidirectional Camera-Ready/resources/ablation_tables.tex <==
\newcommand{\firstwordablationtable}{
    \begin{table*}
    \centering
    \setlength{\tabcolsep}{2pt}
    \fontsize{8}{10}\selectfont
    \begin{tabularx}{\textwidth}{Xrr}
    \toprule[\heavyrulewidth]
                                                              & English-Russian & Russian-English   \\ \hline
    Prompting  ($\text{mT5}_\text{3.7B}$)\\{\tiny Using the full generation from the first time step only -- $G_0$}                                                    & 1.9             & 5.6               \\ \hline
    \textbf{S}equential \textbf{P}rompting ($\text{mT5}_\text{3.7B}$~+~\textsc{Sp}) \\{\tiny Concatenating the full generation at each time step  -- \texttt{CONCAT}($G_0$, \ldots, $G_{t-1}$)}                 & 9.3             & 17.9              \\ \hline
    \textbf{S}equential \textbf{A}utoregressive \textbf{P}rompting ($\text{mT5}_\text{3.7B}$~+~\textsc{Sap}) \\{\tiny Concatenating the first word of the generation at each time step -- \texttt{CONCAT}($F_0$, \ldots, $F_{t-1}$)} & \textbf{20.1}   & \textbf{26.9}     \\ 
    \bottomrule[\heavyrulewidth]
    \end{tabularx}
    \caption{Few-shot (2-shot) machine translation results on FLORES-101 devtest (spBLEU) using $\text{mT5}_{\text{3.7B}}$ as described in Section \ref{sec:few-shot}. In this experiment, over two language pairs, English-Russian and Russian-English, we compare a) simply prompting the model once and taking the full generation $G_0$ b) concatenating the full generation at each time step $G_t$ to the prompt in the next time step c) concatenating just the first word of the generation at each time step $F_t$ to the prompt in the next time step.}
    \label{table:firstword-ablation}
    \end{table*}
}

\newcommand{\mtscoreablationtable}{
    \begin{table}[H]
    \centering
    \begin{tabularx}{\textwidth}{Xrr}
    \toprule[\heavyrulewidth]
                                               & English-Russian & Russian-English \\ \hline
    Random Selection                           & 0.0             & 25.5            \\ 
    mT5Score Filtering and Selection           & \textbf{20.0}   & \textbf{26.3}   \\ 
    \bottomrule[\heavyrulewidth]
    \end{tabularx}
    \caption{Unsupervised zero-shot machine translation results on FLORES-101 devtest (spBLEU) using $\text{mT5}_{\text{3.7B}}$ as described in Section \ref{sec:zero-shot}. In this experiment, we ablate utilizing mT5Score to filter and select the high-quality synthetic examples during bootstrapping over two language pairs, English-Russian and Russian-English. When using random selection, the synthetic parallel examples choosen may be extremely low-quality or non-sensical leading to a 0.0 spBLEU score after self-amplification as shown for the English-Russian language pair. }
    \label{table:mtscore-ablation}
    \end{table}
}

\newcommand{\promptensembleablationtable}{
    \begin{table}[H]
    \centering
    \begin{tabularx}{\textwidth}{Xrr}
    \toprule[\heavyrulewidth]
                                               & English-Russian & Russian-English  \\ \hline
    Single Prompt                              & 20.0           & 26.3              \\
    4 Prompt Ensemble                          & \textbf{20.9}  & 27.9              \\ 
    8 Prompt Ensemble                          & 20.7           & \textbf{28.6}     \\ 
    16 Prompt Ensemble                         & \textbf{20.9}  & \textbf{28.6}     \\ 
    \bottomrule[\heavyrulewidth]
    \end{tabularx}
    \caption{Unsupervised zero-shot machine translation results on FLORES-101 devtest (spBLEU) using $\text{mT5}_{\text{3.7B}}$ as described in Section \ref{sec:zero-shot}. In this experiment, we compare utilizing a single few-shot prompt with two synthetic parallel examples to perform the final translation with utilizing an ensemble of 4, 8, and 16 distinct few-shot prompts each with two synthetic parallel examples that generate 4, 8, and 16 translations respectively from which the best translation (by mT5Score) is selected as the final translation over two language pairs, English-Russian and Russian-English.}
    \label{table:promptensemble-ablation}
    \end{table}
}




\newcommand{\englishcentricablationtable}{
    \begin{table}[H]
    \centering
    \begin{tabularx}{\textwidth}{Xrrr}
    \toprule[\heavyrulewidth]
                                & English-Russian & Russian-Chinese   \\ \hline
    Standard bootstrap          & 20.9            & 5.8              \\ 
    English-centric bootstrap   & \textbf{21.2}   & \textbf{8.3}     \\ 
    \bottomrule[\heavyrulewidth]
    \end{tabularx}
    \caption{Unsupervised zero-shot machine translation results on FLORES-101 devtest (spBLEU) using $\text{mT5}_{\text{3.7B}}$ as described in Section \ref{sec:zero-shot}. In this experiment, we ablate utilizing the English-centric bootstrap described in Section \ref{sec:englishcentric} over two language pairs, English-Russian and Russian-Chinese.}
    \label{table:englishcentric-ablation}
    \end{table}
}

\newcommand{\selfampablationtable}{
    \begin{table}[H]
    \centering
    \begin{tabularx}{\textwidth}{Xrr}
    \toprule[\heavyrulewidth]
                                               & English-Russian & Russian-English \\ \hline
    Standard                                   & 0.4             & 4.6            \\ 
    Bootstrapping and self-amplification       & \textbf{21.2}   & \textbf{27.9}   \\ 
    \bottomrule[\heavyrulewidth]
    \end{tabularx}
    \caption{Unsupervised zero-shot machine translation results on FLORES-101 devtest (spBLEU) using $\text{mT5}_{\text{3.7B}}$ as described in Section \ref{sec:zero-shot}. In this experiment, we compare the standard zero-shot performance of mT5 with \textsc{Sap} against the zero-shot performance achievable implementing the bootstrapping and self-amplification techniques from \citet{gpt3unsupervised} with the adaptations described in Section \ref{sec:zero-shot}. }
    \label{table:selfamp-ablation}
    \end{table}
}

==> Bidirectional Camera-Ready/resources/few-shot_results.tex <==
\newcommand{\hlinep}{
    \hline & \\[-1.5ex]
}

\newcommand{\fewshotfloresresultstablerow}[7]{
    \multirow{5}{*}{#1}  & Supervised &                                \xintFor ##8 in #2 \do {  & ##8 }    \\ 
                         & $\text{GPT-3}_{\text{6.7B}}$ & (32\text{-shot})   \xintFor ##8 in #3 \do {  & ##8 }    \\
                         & $\text{XGLM}_{\text{7.5B}}$ & (32\text{-shot})    \xintFor ##8 in #4 \do {  & ##8 }    \\
                         & $\text{mT5}_{\text{3.7B}}\ + \  \text{\textsc{Sap}}$ & (2\text{-shot})      \xintFor ##8 in #5 \do {  & ##8 }    \\
                         & $\text{mT5}_{\text{3.7B}}\ + \  \text{\textsc{Sap}}$ &  (zero\text{-shot})  \xintFor ##8 in #6 \do {  & ##8 }  \\
                         #7
}

\newcommand{\fewshotfloresresultstable}{
    \begin{table}[H]
    % \vspace{-13.3em}%
    \centering
    \fontsize{6}{6}\selectfont
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{llrcccccccccccccc|c}
    \toprule[\heavyrulewidth]
                         & &                                 & en & de & fr & ca & fi & ru & bg & zh & ko & ar & sw & hi & my & ta & avg \\ \hlinep
    \fewshotfloresresultstablerow{en}
        {{–,32.6,42.0,31.2,24.2,27.1,37.4,19.3,18.5,17.9,26.9,28.1,3.5,3.4,24.0}}
        {{–,25.9,\textbf{36.1},23.8,10.2,11.2,5.9,12.5,1.2,1.1,0.5,0.3,0.1,0.0,9.9}}
        {{–,\textbf{27.6},36.0,\underline{\textbf{34.0}},\textbf{23.3},\textbf{24.2},\textbf{33.1},\textbf{15.6},\textbf{12.0},11.5,18.0,\textbf{19.9},\underline{11.0},\underline{8.5},\textbf{21.1}}}
        {{–,23.2,34.2,26.2,15.8,20.1,27.9,9.5,10.4,11.4,17.3,14.0,\underline{11.0},\underline{11.2},17.9}}
        {{–,26.0,33.2,28.4,15.7,21.2,27.1,11.3,10.5,\textbf{12.7},\textbf{19.1},16.1,\underline{\textbf{13.2}},\underline{\textbf{13.1}},19.0}}{\hlinep}

    \fewshotfloresresultstablerow{de}
        {{35.8,–,35.5,25.8,22.6,24.6,31.5,17.2,16.6,14.8,21.0,23.4,2.3,2.3,21.0}}
        {{\underline{\textbf{40.4}},–,26.2,17.2,8.1,9.3,4.8,9.0,1.0,0.9,0.5,0.3,0.1,0.1,9.1}}
        {{\underline{38.8},–,\textbf{27.9},19.1,\textbf{20.5},\textbf{19.7},\textbf{25.8},\textbf{12.3},3.4,6.6,11.7,\textbf{14.3},\underline{\textbf{9.9}},\underline{4.8},\textbf{16.5}}}
        {{33.0,–,24.4,17.8,14.1,15.7,20.2,8.2,\textbf{9.1},7.7,11.0,10.0,\underline{9.8},\underline{9.6},14.7}}
        {{\underline{35.9},–,25.9,\textbf{22.5},14.3,17.4,21.0,8.2,8.4,\textbf{8.7},\textbf{13.4},10.4,\underline{9.0},\underline{\textbf{10.8}},15.8}}{\hlinep}

    \fewshotfloresresultstablerow{fr}
        {{37.2,28.5,–,28.7,21.9,24.5,32.2,17.6,16.7,15.4,17.2,22.9,2.1,0.8,20.4}}
        {{\underline{\textbf{42.8}},20.9,–,23.7,8.0,9.7,4.6,9.1,1.0,1.0,0.4,0.3,0.1,0.0,9.4}}
        {{\underline{40.4},20.4,–,\underline{\textbf{32.1}},\textbf{19.4},\textbf{19.8},\textbf{26.3},\textbf{10.6},2.4,5.9,14.5,\textbf{13.7},\underline{9.7},\underline{6.6},\textbf{17.1}}}
        {{\underline{38.0},19.2,–,26.7,13.7,18.3,23.5,8.6,\textbf{9.2},9.9,15.0,12.1,\underline{\textbf{10.8}},\underline{9.7},16.5}}
        {{\underline{38.1},\textbf{21.1},–,\underline{30.1},12.9,18.1,22.3,8.7,\textbf{9.2},\textbf{11.1},\textbf{15.7},11.0,\underline{9.6},\underline{\textbf{11.1}},16.8}}{\hlinep}

    \fewshotfloresresultstablerow{ca}
        {{33.4,24.8,35.1,–,19.0,21.1,28.6,15.1,13.9,13.4,18.7,20.5,2.1,2.6,19.1}}
        {{\underline{40.2},18.6,31.4,–,7.0,9.3,4.3,8.0,0.9,0.9,0.3,0.4,0.1,0.1,9.3}}
        {{\underline{\textbf{41.1}},18.9,\textbf{33.8},–,11.3,3.3,\textbf{23.9},\textbf{10.8},1.3,0.8,13.8,6.1,\underline{7.9},\underline{3.1},13.6}}
        {{\underline{33.4},14.9,29.5,–,10.7,14.0,15.6,6.5,7.0,5.6,12.4,7.3,\underline{\textbf{8.7}},\underline{6.7},13.3}}
        {{\underline{37.1},\textbf{19.3},32.4,–,\textbf{12.4},\textbf{16.7},19.1,7.9,\textbf{7.4},\textbf{8.5},\textbf{14.5},\textbf{9.4},\underline{8.3},\underline{\textbf{9.8}},\textbf{15.6}}}{\hlinep}

    \fewshotfloresresultstablerow{fi}
        {{27.2,23.0,29.3,21.6,–,20.6,26.4,16.0,14.8,12.4,14.2,19.8,1.7,0.9,17.5}}
        {{25.3,13.5,17.1,10.0,–,6.4,2.8,5.7,0.7,0.7,0.3,0.3,0.1,0.0,6.4}}
        {{\underline{\textbf{29.2}},\textbf{17.4},\textbf{22.2},\textbf{17.0},–,\textbf{16.5},\textbf{17.5},\textbf{12.4},\textbf{7.5},\textbf{7.6},8.0,\textbf{10.1},\underline{6.2},\underline{2.0},\textbf{13.4}}}
        {{24.1,16.1,19.8,14.9,–,14.2,17.0,7.0,5.8,7.1,8.3,5.6,\underline{\textbf{8.5}},\underline{3.9},11.7}}
        {{23.2,16.1,20.5,16.3,–,14.5,16.3,8.0,5.9,6.3,\textbf{10.0},7.5,\underline{5.9},\underline{\textbf{8.2}},12.2}}{\hlinep}

    \fewshotfloresresultstablerow{ru}
        {{27.5,23.5,30.1,22.0,19.4,–,31.0,16.5,15.3,13.5,18.1,20.9,2.2,2.3,18.6}}
        {{\underline{28.1},14.8,20.4,13.1,5.4,–,7.4,1.2,0.2,0.2,0.1,0.2,0.1,0.1,7.0}}
        {{\underline{\textbf{30.4}},\textbf{17.9},\textbf{24.0},14.6,8.0,–,\textbf{26.3},\textbf{11.6},5.5,7.4,7.1,\textbf{9.1},\underline{7.3},\underline{3.1},13.2}}
        {{26.9,16.6,22.4,14.5,11.2,–,25.2,6.1,8.0,6.4,11.3,\textbf{9.1},\underline{\textbf{9.8}},\underline{8.4},13.5}}
        {{\underline{27.9},17.1,22.5,\textbf{19.4},\textbf{13.1},–,25.4,8.3,\textbf{8.7},\textbf{9.1},\textbf{12.0},9.0,\underline{9.0},\underline{\textbf{10.3}},\textbf{14.8}}}{\hlinep}

    \fewshotfloresresultstablerow{bg}
        {{33.0,26.1,33.7,24.9,20.8,26.5,–,17.5,16.4,14.5,20.9,23.1,2.3,2.4,20.2}}
        {{21.6,11.4,16.0,9.7,4.3,6.5,–,1.2,0.2,0.2,0.1,0.2,0.1,0.1,5.5}}
        {{\underline{\textbf{35.5}},\textbf{19.2},\textbf{26.3},12.9,\textbf{14.2},22.9,–,\textbf{11.9},6.8,\textbf{9.2},9.4,7.5,\underline{3.2},1.0,13.9}}
        {{31.0,17.0,23.8,18.3,10.9,22.9,–,7.2,\textbf{8.3},8.1,11.7,7.4,\underline{\textbf{9.5}},\underline{6.6},14.1}}
        {{32.5,17.3,24.5,\textbf{21.7},10.6,\textbf{23.2},–,8.7,7.5,9.0,\textbf{13.0},\textbf{8.6},\underline{7.9},\underline{\textbf{10.1}},\textbf{15.0}}}{\hlinep}

    \fewshotfloresresultstablerow{zh}
        {{20.9,17.6,24.3,17.4,16.0,17.2,22.1,–,15.9,11.6,15.5,18.5,1.9,2.5,15.5}}
        {{\underline{\textbf{21.1}},9.5,14.3,8.2,4.3,3.6,1.3,–,1.1,0.4,0.2,0.2,0.1,0.0,4.9}}
        {{20.7,8.3,8.5,10.5,4.4,4.8,\textbf{14.8},–,\textbf{9.3},4.2,5.6,\textbf{12.0},\underline{8.6},\underline{6.2},9.1}}
        {{19.0,\textbf{10.9},\textbf{14.9},11.9,8.0,10.6,11.9,–,8.9,6.0,\textbf{9.1},8.0,\underline{\textbf{10.0}},\underline{7.6},10.5}}
        {{18.5,\textbf{10.9},14.8,\textbf{12.8},\textbf{8.8},\textbf{10.7},11.8,–,9.2,\textbf{6.5},9.0,8.9,\underline{8.2},\underline{\textbf{8.9}},\textbf{10.7}}}{\hlinep}

    \fewshotfloresresultstablerow{ko}
        {{20.9,16.7,22.1,16.5,14.9,15.5,21.1,15.7,–,10.6,15.1,18.7,1.9,4.0,14.9}}
        {{8.3,4.6,6.4,4.4,2.1,1.7,0.8,2.5,–,0.2,0.1,0.1,0.1,0.1,2.4}}
        {{\textbf{19.9},\textbf{10.3},13.7,5.3,1.4,1.2,10.9,\textbf{11.9},–,2.7,3.2,1.0,\underline{2.2},1.4,6.5}}
        {{18.3,10.1,13.7,11.3,\textbf{7.9},\textbf{10.1},\textbf{12.6},7.8,–,\textbf{6.3},7.2,6.6,\underline{2.6},\underline{4.7},9.2}}
        {{18.1,10.1,\textbf{13.8},\textbf{12.8},7.8,9.9,11.4,7.6,–,5.5,\textbf{8.0},\textbf{6.7},\underline{\textbf{8.1}},\underline{\textbf{8.2}},\textbf{9.8}}}{\hlinep}

    \fewshotfloresresultstablerow{ar}
        {{25.5,18.7,25.7,18.9,15.6,17.8,23.8,13.1,13.3,–,15.4,19.4,1.8,0.9,16.1}}
        {{10.5,5.3,9.6,6.0,2.2,2.2,0.9,0.9,0.1,–,0.1,0.1,0.2,0.0,2.9}}
        {{\underline{\textbf{27.7}},\textbf{12.2},17.9,8.8,\textbf{8.5},9.1,\textbf{18.4},\textbf{8.9},0.8,–,7.7,7.8,\underline{3.4},\underline{3.7},10.4}}
        {{23.7,10.8,17.5,11.0,8.0,12.2,13.8,5.9,7.1,–,10.3,\textbf{8.0},\underline{8.0},\underline{8.0},11.1}}
        {{\underline{26.9},11.5,\textbf{19.8},\textbf{15.9},7.8,\textbf{14.5},13.6,6.3,\textbf{7.6},–,\textbf{11.0},\textbf{8.0},\underline{\textbf{8.8}},\underline{\textbf{9.3}},\textbf{12.4}}}{\hlinep}

    \fewshotfloresresultstablerow{sw}
        {{30.4,19.4,26.7,20.1,15.6,17.6,23.8,13.2,12.2,12.0,–,19.2,2.1,4.0,16.6}}
        {{5.0,2.9,3.9,2.8,1.7,1.8,1.3,1.3,0.5,0.5,–,0.4,0.1,0.1,1.7}}
        {{\underline{\textbf{31.6}},13.4,\textbf{21.8},15.4,\textbf{10.2},13.1,15.2,\textbf{9.5},\textbf{6.0},\textbf{8.9},–,\textbf{7.6},\underline{3.4},1.0,\textbf{12.1}}}
        {{27.0,12.6,19.0,15.1,9.2,12.2,\textbf{15.8},5.9,\textbf{6.0},8.3,–,6.5,\underline{\textbf{5.4}},\underline{6.0},11.5}}
        {{30.0,\textbf{13.5},20.0,\textbf{18.0},9.5,\textbf{14.5},\textbf{15.8},6.9,5.7,7.7,–,6.5,\underline{2.7},\underline{\textbf{7.0}},\textbf{12.1}}}{\hlinep}

    \fewshotfloresresultstablerow{hi}
        {{27.9,19.4,25.9,18.9,15.7,16.9,23.9,13.5,13.9,12.2,16.8,–,2.5,3.8,16.2}}
        {{1.2,0.9,1.4,0.8,0.4,0.4,0.3,0.2,0.1,0.1,0.1,–,0.1,0.2,0.5}}
        {{25.2,12.3,15.4,8.8,\textbf{9.8},11.5,11.3,\textbf{10.8},\textbf{8.5},6.1,4.7,–,1.5,1.9,9.8}}
        {{25.7,12.4,17.0,13.0,8.0,12.2,\textbf{15.4},7.2,4.4,7.4,\textbf{8.9},–,\underline{9.6},\underline{9.0},11.6}}
        {{\textbf{27.1},\textbf{12.6},\textbf{17.3},\textbf{14.3},9.0,\textbf{12.4},14.5,8.0,6.7,\textbf{8.1},\textbf{8.9},–,\underline{\textbf{10.2}},\underline{\textbf{12.8}},\textbf{12.5}}}{\hlinep}

    \fewshotfloresresultstablerow{my}
        {{10.0,6.9,10.4,8.5,6.0,6.7,9.5,5.7,6.1,4.6,7.2,9.1,–,2.5,7.2}}
        {{0.5,0.3,0.4,0.4,0.2,0.1,0.2,0.0,0.0,0.0,0.1,0.2,–,0.1,0.2}}
        {{\underline{14.1},\underline{7.6},10.1,3.8,5.7,\underline{7.1},8.9,\underline{\textbf{7.1}},\underline{\textbf{6.9}},3.6,3.5,\textbf{8.9},–,\underline{2.6},6.9}}
        {{\underline{\textbf{16.8}},\underline{8.5},\underline{\textbf{12.9}},\underline{11.0},\underline{6.7},6.1,9.2,5.2,2.9,\underline{\textbf{5.0}},\underline{\textbf{8.0}},7.0,–,\underline{5.7},\underline{8.1}}}
        {{\underline{16.4},\underline{\textbf{9.0}},\underline{11.9},\underline{\textbf{11.6}},\underline{\textbf{6.9}},\underline{\textbf{8.3}},\underline{\textbf{10.4}},5.5,3.6,\underline{4.8},6.4,7.1,–,\underline{\textbf{6.2}},\underline{\textbf{8.3}}}}{\hlinep}

    \fewshotfloresresultstablerow{ta}
        {{8.3,4.9,6.8,5.8,5.0,4.7,7.0,2.5,2.3,1.1,5.2,6.9,1.2,–,4.8}}
        {{1.0,0.5,0.8,0.5,0.2,0.3,0.3,0.1,0.2,0.1,0.1,0.2,0.0,–,0.3}}
        {{\underline{16.3},\underline{8.4},\underline{10.3},5.1,\underline{5.2},\underline{8.1},\underline{7.6},\underline{\textbf{8.1}},\underline{6.2},\underline{5.4},2.8,\underline{7.2},0.9,–,\underline{7.1}}}
        {{\underline{18.7},\underline{10.4},\underline{13.7},\underline{10.9},\underline{6.3},\underline{9.8},\underline{11.6},\underline{5.2},0.7,\underline{6.5},\underline{6.0},\underline{9.3},\underline{1.8},–,\underline{8.5}}}
        {{\underline{\textbf{20.4}},\underline{\textbf{10.5}},\underline{\textbf{14.7}},\underline{\textbf{12.9}},\underline{\textbf{8.1}},\underline{\textbf{10.6}},\underline{\textbf{13.2}},\underline{7.0},\underline{\textbf{6.8}},\underline{\textbf{6.6}},\underline{\textbf{8.3}},\underline{\textbf{10.1}},\underline{\textbf{2.6}},–,\underline{\textbf{10.1}}}}{\hlinep}

    \fewshotfloresresultstablerow{avg}
        {{26.0,20.2,26.7,20.0,16.7,18.5,24.5,14.1,13.5,11.8,16.3,19.3,2.1,2.5,16.6}}
        {{18.9,9.9,14.2,9.3,4.2,4.8,2.7,4.0,0.6,0.5,0.2,0.3,0.1,0.1,5.0}}
        {{\underline{\textbf{28.5}},14.9,20.6,14.4,\textbf{10.9},12.4,\textbf{18.5},\textbf{10.9},5.9,6.1,8.5,\textbf{9.7},\underline{5.8},\underline{3.5},12.2}}
        {{25.8,14.1,20.2,15.6,10.0,13.7,16.9,6.9,6.8,7.4,10.5,8.5,\underline{\textbf{8.1}},\underline{7.5},12.3}}
        {{\underline{27.1},\textbf{15.0},\textbf{20.9},\textbf{18.2},10.5,\textbf{14.8},17.1,7.9,\textbf{7.5},\textbf{8.0},\textbf{11.5},9.2,\underline{8.0},\underline{\textbf{9.7}},\textbf{13.2}}}{}
    \bottomrule[\heavyrulewidth]
    \end{tabular}
    \caption{Few-shot and unsupervised zero-shot machine translation results on FLORES-101 devtest (spBLEU). Source language in rows, target language in columns. $\text{GPT-3}_{\text{6.7B}}$ and $\text{XGLM}_{\text{7.5B}}$ use 32 examples from the dev set for few-shot learning. $\text{mT5}_{\text{3.7B}}$ uses 2 examples from the dev set for few-shot learning. Supervised results correspond to the M2M-124 615M model from \citet{flores101}. $\text{XGLM}_{\text{7.5B}}$ results correspond to the model from \citet{xglm}. Underline denotes better than supervised, bold denotes best of \text{GPT-3}, XGLM, and mT5. spBLEU computed using the implementation from \citet{flores101}.} 
    \label{table:fewshot-flores-results}
    \end{table}
}


\newcommand{\fewshotfloresresultstableabbrev}{
    \begin{table*}
    \centering
    \small
    %\vspace{-60em}%
    \begin{tabular}{lrrrrr|r}
    \toprule[\heavyrulewidth]
                                                         && HR~$\rightarrow$~HR & LR~$\rightarrow$~HR & HR~$\rightarrow$~LR & LR~$\rightarrow$~LR & All   \\ \hline
    Number of Language Pairs & & 110 & 33 & 33 & 6 & 182 \\ \hline
    $\text{Supervised}$            &                                  & 21.5 & 10.3 & 8.6 & 4.3  & 16.6    \\ 
    $\text{GPT-3}_{\text{6.7B}}$ & (32\text{-shot})                   & 8.1 & 0.4 & 0.1 & 0.1  & 5.0    \\ 
    $\text{XGLM}_{\text{7.5B}}$ & (32\text{-shot})                    & 15.3 & 8.7 & 6.8 & 3.8  & 12.2             \\ 
    $\text{mT5}_{\text{3.7B}}\ + \  \text{\textsc{Sap}}$ & (2\text{-shot})     & 14.5 & 9.8 & 8.2 & 7.1  & 12.3             \\ 
    $\text{mT5}_{\text{3.7B}}\ + \  \text{\textsc{Sap}}$ & (zero\text{-shot})  & \textbf{15.5} & \textbf{10.7} & \textbf{9.1} & \textbf{8.2} & \textbf{13.2}            \\
    \bottomrule[\heavyrulewidth]
    \end{tabular}
    \caption{Abbreviated few-shot and unsupervised zero-shot machine translation results on FLORES-101 devtest (spBLEU). The matrix of full results can be found in Appendix \ref{sec:flores-results}. Results are average spBLEU scores over subsets of the 182 language pairs (\texttt{src}~$\rightarrow~$\texttt{tgt}) where ``LR'' is a low-resource language and ``HR'' is a high-resource language. ``All'' represents the average spBLEU score over all 182 language pairs. Supervised results correspond to the M2M-124 615M model from \citet{flores101}. $\text{XGLM}_{\text{7.5B}}$ results correspond to the model from \citet{xglm}. Bold denotes best of \text{GPT-3}, XGLM, and mT5. spBLEU computed using the implementation from \citet{flores101}.}
    \label{table:fewshot-flores-results-abbrev}
    \end{table*}
}

==> Bidirectional Camera-Ready/resources/figures.tex <==
\newcommand{\fewshotfigure}{
    \begin{figure}[t]
        \centering
        \includegraphics[width=400px]{few-shot-long}
        \caption{A visualization of our \textsc{Sap} technique extracting high-quality translations from mT5. In the zero-shot setting, the examples used in the prompt are synthetic examples retrieved in a fully unsupervised manner.}
        \label{fig:fewshot}
    \end{figure}
}

\newcommand{\bootstrapfigure}{
    \begin{figure*}
        \centering
        \includegraphics[width=400px]{bootstrap}
        \caption{A visualization of the bootstrapping process described in Section \ref{sec:zero-shot}. }
        \label{fig:bootstrap}
    \end{figure*}
}

==> Bidirectional Camera-Ready/resources/selected_generations.tex <==
\newcommand{\exampleMT}[9]{
\vspace{1em}
\noindent\underline{Task:} #1-shot Machine Translation (Example \##2) \\
\\ \underline{Dataset:} FLORES-101 (#3~$\rightarrow$~#4) \\
\\ \underline{Prompt Template:} \\ \\
\texttt{\small{Translate #3 to #4.\\
\ifthenelse{\equal{#1}{Few}}{{\{\{examples\}\}\\}}{{}}
#3: \{\{source\_text\}\}\\
#4: }}
%\\ \\ \underline{Source Text:} \\ \\
%\texttt{\small{#5}}
\\ \\ \underline{Ground Truth:} \\ \\
\texttt{\small{#6}}
\\ \\ \underline{Generation ($\text{mT5}_\text{3.7B}$~+~\textsc{Sap}):} \\ \\
\texttt{\small{#7}}
\\ \\ \underline{Generation ($\text{mT5}_\text{3.7B}$):} \\ \\
\texttt{\small{#8}}
\\ \\ \underline{Commentary:} \\ \\
#9
\raggedbottom
\pagebreak
}

\newcommand{\exampleQA}[9]{
\vspace{1em}
\noindent\underline{Task:} #1-shot Question Answering (Example \##2) \\
\\ \underline{Dataset:} #3 \\
\\ \underline{Prompt Template:} \\ \\
\texttt{\small{Answer the question based on the following passage.\\\\
\ifthenelse{\equal{#1}{Few}}{{\{\{examples\}\}\\\\}}{{}}
Passage: \{\{passage\}\}\\
Question: \{\{question\}\}\\
Answer: }}
\\ \\ \underline{Passage:} \\ \\
\texttt{\small{#4}}
\\ \\ \underline{Question:} \\ \\
\texttt{\small{#5}}
\\ \\ \underline{Ground Truth:} \\ \\
\texttt{\small{#6}}
\\ \\ \underline{Generation ($\text{mT5}_\text{3.7B}$~+~\textsc{Sap}):} \\ \\
\texttt{\small{#7}}
\\ \\ \underline{Generation ($\text{mT5}_\text{3.7B}$):} \\ \\
\texttt{\small{#8}}
\\ \\ \underline{Commentary:} \\ \\
#9
\raggedbottom
\pagebreak
}

\newcommand{\exampleSUM}[6]{
\vspace{1em}
\noindent\underline{Task:} Few-shot Summarization (Example \##1) \\
\\ \underline{Dataset:} CNN / Daily Mail v3.0.0 \\
\\ \underline{Prompt Template:} \\ \\
\texttt{\small{Summarize the article.\\\\
\{\{examples\}\}\\\\
Article: \{\{article\}\}\\
Summary: }}
\\ \\ \underline{Article:} \\ \\
\texttt{\small{#2}}
\\ \\ \underline{Summary:} \\ \\
\texttt{\small{#3}}
\\ \\ \underline{Generation ($\text{mT5}_\text{3.7B}$~+~\textsc{Sap}):} \\ \\
\texttt{\small{#4}}
\\ \\ \underline{Generation ($\text{mT5}_\text{3.7B}$):} \\ \\
\texttt{\small{#5}}
\\ \\ \underline{Commentary:} \\ \\
#6
\raggedbottom
\pagebreak
}



\newcommand{\selectedgenerations} {

\exampleMT{Few}
{1}
{Arabic}
{English}
{
}
{The 802.11n standard operates on both the 2.4Ghz and 5.0Ghz frequencies.}
{The wireless standard 802.11n operates at the frequency of 2.4 GHz and 5 GHz.}
{The 802.11n wireless standard operates at 2.4 and 5.0}
{\textsc{Sap} generates a lengthier and more fluent translation and correctly translates the units of the frequencies. Both generations add the word ``wireless'' which is used correctly and is likely to appear next to the words ``802.11n'' and ``standard'' but does not exist in the ground truth translation.}

\exampleMT{Few}
{2}
{Russian}
{English}
{}
{In 1956 Słania moved to Sweden, where three years later he began work for the Swedish Post Office and became their chief engraver.}
{In 1956, Slania moved to Sweden, where he worked for three years for the Swedish Post Office and became its chief engraved worker.}
{In 1956, Slanya moved to Sweden and became...}
{\textsc{Sap} generates a full length translation and more correctly translates ``Słania'' to ``Slania'' instead of ``Slanya''. While the translation without \textsc{Sap} only generates a partial translation, the word ``became'' indicates the direction of translation would be less close to the ground truth translation than the direction of translation taken by \textsc{Sap}. Notably, \textsc{Sap} produces a relatively high-quality translation, but a common failure mode is displayed in this example. \textsc{Sap} translates ``chief  engraver'' to ``chief engraved worker'' which is an imperfect paraphrase likely due to an imperfect multilingual alignment of the word  ``engraver'' in the embedding space of the model.}

\exampleQA{Few}
{1}
{SQuAD v1.1}
{In 1874, Tesla evaded being drafted into the Austro-Hungarian Army in Smiljan by running away to Tomingaj, near Gračac. There, he explored the mountains in hunter's garb. Tesla said that this contact with nature made him stronger, both physically and mentally. He read many books while in Tomingaj, and later said that Mark Twain's works had helped him to miraculously recover from his earlier illness.}
{Why did Tesla avoid by fleeing Smiljan?}
{being drafted into the Austro-Hungarian Army}
{because he was ill and wanted to avoid being drafted into the Austro-Hungarian Army}
{because he was ill and could not leave the country}
{In this example, the grammaticality of the question itself (``\textit{Why} did Tesla avoid by fleeing Smiljan?'' vs. ``\textit{What} did Tesla avoid by fleeing Smiljan?'') has issues. This seems to cause both generations to attempt to answer a ``why'' style question with ``because'' instead of a ``what'' style question. Notably, the answer generated by \textsc{Sap} does eventually reach correct answer where as the the answer generated without \textsc{Sap} hallucinates a fact: ``he [Tesla] \ldots could not leave the country''.}

\exampleQA{Few}
{2}
{SQuAD v1.1}
{The Broncos took an early lead in Super Bowl 50 and never trailed. Newton was limited by Denver's defense, which sacked him seven times and forced him into three turnovers, including a fumble which they recovered for a touchdown. Denver linebacker Von Miller was named Super Bowl MVP, recording five solo tackles, 2½ sacks, and two forced fumbles.}
{Who won the MVP for the Super Bowl?}
{Von Miller}
{Von Miller}
{Von Miller, Denver, NFL, NFLPA}
{Without using \textsc{Sap}, the answer generated is correct, but contains hallucinated tokens towards the end of the generation.}

\exampleSUM{1}
{London (CNN)The Hatton Garden heist, as it will surely come to be known, was every safe deposit box holder's nightmare, every movie director's dream. Thieves using heavy cutting equipment and rappelling gear broke into the vault of an esteemed 60-year-old safe deposit company in the heart of London over the past holiday weekend, possibly taking advantage of as many as four days to rifle through an uncounted number of safe deposit boxes. And they reportedly got away with hundreds of thousands of pounds worth of gems and cash -- even, in the educated guess of one former police official, as much as 200 million pounds, or\ldots[truncated]}
{Robbers may have taken advantage of a four-day holiday weekend. Estimates of the value of the items taken rage from hundreds of thousands of pounds to 200 million pounds. The heist took place in a historic heart of London's jewelry business.}
{The Hatton Garden heist was a nightmare for jewelers and their customers. They were 'treated like criminals', while officers said they would double bail for anyone who was arrested before. They were arrested while on the sidewalk .}
{The latest jewel heist in London took place over the weekend.}
{\textsc{Sap} generates a lengthier generation with multiple sentences summarizing the article. Some of the facts presented in the generation, however, are not coherent with the article.}

\exampleSUM{2}
{Sanaa, Yemen (CNN)Al Qaeda fighters attacked a prison in the coastal Yemeni city of Al Mukallah early Thursday, freeing at least 270 prisoners, a third of whom have al Qaeda links, a senior Defense Ministry official has told CNN. Khaled Batarfi, a senior al Qaeda figure, was among the escapees, officials said. Dozens of attackers took control of government buildings, including the city's Central Prison, Central Bank and radio station during the assault early Thursday, according to officials. Government troops arrived early Thursday and clashed with the al Qaeda fighters, and most of the militants fled,\ldots[truncated]}
{Al Qaeda fighters attack a prison and other government buildings, freeing many prisoners. Government troops clash with the fighters, most of whom flee. Yemen is descending into chaos as a Shia-Sunni conflict draws in regional rivals Saudi Arabia and Iran.}
{Yemen's al Qaeda fighters escape from prison after clash with government forces.}
{Yemen's prisoners escape from al Qaeda fighting in Yemen}
{\textsc{Sap} correctly characterizes the major theme of the article in its summary. Without \textsc{Sap}, the generation devolves in to an incoherent fact (``prisoners escape from al Qaeda fighting'') and only a partial summary is generated. The ground truth summary, however, is notably longer and contains multiple sentences, while the summary generated by \textsc{Sap} in this instance is only a single sentence.}

}

==> Bidirectional Camera-Ready/resources/squad_and_summarization_results.tex <==
\newcommand{\squadandsummarizationtable}{
    \begin{table}[t]
    \centering
    \captionsetup{justification=centering}
    \setlength{\tabcolsep}{3pt}
    \small
    %\vspace{-60em}%

    % SQUAD
    \begin{minipage}[t]{0.42\linewidth}\centering
        \fontsize{8}{9}\selectfont
        \begin{tabular}{llrrr}
            \toprule[\heavyrulewidth]
                                                                                 && EM              & F1             \\ \hline
            \textit{Zero-shot}                                                                                       \\ \hline 
            $\text{T5+LM}_{\text{3B}}$                     & (zero\text{-shot})   & 23.5            & 48.4           \\ 
            $\text{mT5}_{\text{3.7B}}$ $+$ \ $\text{\textsc{Sap}}$  & (zero\text{-shot})   & \textbf{30.2}    & \textbf{54.0} \\ \hline
            \textit{Few-shot}                                                                                        \\ \hline   
            $\text{mT5}_{\text{3.7B}}$\                    & (16\text{-shot})     & 23.0            & 54.5            \\ 
            $\text{mT5}_{\text{3.7B}}$\ $+$ \ $\text{\textsc{Sap}}$ & (16\text{-shot})     & \textbf{35.4}   & \textbf{60.0}   \\ 
            \bottomrule[\heavyrulewidth]
        \end{tabular}
        \caption{Zero-shot and few-shot question answering results on the SQuAD v1.1 dev set \citep{squad}.}
        \label{table:squad}
    \end{minipage}\hfill%
    % Summarization
    \begin{minipage}[t]{0.57\linewidth}\centering
        \fontsize{8}{9}\selectfont
        \begin{tabular}{llrrr}
        \toprule[\heavyrulewidth]
                                                                          && ROUGE-1         & ROUGE-2        & ROUGE-L      \\ \hline
        \textit{Zero-shot}                                                                                       \\ \hline 
        $\text{T5+LM}_{\text{3B}}$ & (zero\text{-shot})                       &  5.3            &  0.6            &  4.9         \\ 
        $\text{mT5}_{\text{3.7B}}$ & (zero\text{-shot})                       & 15.4            & 4.6            & 14.5         \\ 
        $\text{mT5}_{\text{3.7B}}$\ $+$ \ $\text{\textsc{Sap}}$ & (zero\text{-shot})   & \textbf{22.0}   & \textbf{7.4}   & \textbf{20.1} \\ \hline
        \textit{Few-shot}                                                                                       \\ \hline 
        $\text{T5+LM}_{\text{3B}}$ & (2\text{-shot})                       & 14.1            & 4.4            & 13.2         \\ 
        $\text{mT5}_{\text{3.7B}}$ & (2\text{-shot})                       & 15.9            & 4.5            & 15.0         \\ 
        $\text{mT5}_{\text{3.7B}}$\ $+$ \ $\text{\textsc{Sap}}$ & (2\text{-shot})   & \textbf{22.0}   & \textbf{6.8}   & \textbf{20.3} \\ 
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        \caption{Zero-shot and few-shot summarization results on the CNN / Daily Mail v3.0.0 test set evaluated with ROUGE \citep{cnndailymail,cnndailymail2,cnndailymail3,rouge}.}
        \label{table:summarization}
    \end{minipage}
    \end{table}
}

==> Bidirectional Camera-Ready/resources/xquad_results.tex <==
\newcommand{\xquadtable}{
    \begin{table*}
    \fontsize{6}{9}\selectfont
    \centering
    \setlength{\tabcolsep}{2pt}
    %\vspace{-60em}%
    \begin{tabular}{llccccccccccc|c}
    \toprule[\heavyrulewidth]
                                                                         && en      & ar      & de      & el      & es      & hi      & ru      & th      & tr      & vi      & zh      & avg  \\ \hline
    $\text{XGLM}_{\text{7.5B}}$ & (\text{zero-shot})                      & 19.5/31.9 & 12.9/29.6 & 12.2/25.3 & 7.2/28.2 & 12.5/24.0 & \textbf{11.0}/14.0 & 10.9/27.8 & \textbf{16.8}/\textbf{26.4} & 13.6/26.8 & 12.5/21.2 & 13.2/20.3 & 12.9/25.0 \\
    $\text{mT5}_{\text{3.7B}}$\ $+$ \ $\text{\textsc{Sap}}$ & (\text{zero-shot})   & \textbf{25.0}/\textbf{48.8} & \textbf{17.4}/\textbf{39.4} & \textbf{19.4}/\textbf{43.0} & \textbf{9.7}/\textbf{41.0} & \textbf{15.0}/\textbf{42.1} & 6.6/\textbf{32.1} & \textbf{16.1}/\textbf{39.0} & 2.8/17.4 & \textbf{15.8}/\textbf{37.0} & \textbf{18.2}/\textbf{41.9} & \textbf{15.0}/\textbf{29.0} & \textbf{14.6}/\textbf{37.3} \\
    \bottomrule[\heavyrulewidth]
    \end{tabular}
    \caption{Zero-shot multilingual question answering results (EM/F1) on the XQuAD test set \citep{xquad}.}
    \label{table:xquad}
    \end{table*}
}

==> Bidirectional Camera-Ready/resources/zero-shot_results.tex <==
\newcommand{\selfamplificationtable}{
    \begin{table}[H]
    \centering
    %\vspace{-60em}%
    \begin{tabularx}{\textwidth}{lXrr}
    \toprule[\heavyrulewidth]
                                                                                         && English-French  & French-English  \\ \hline
    $\text{GPT-3}_{\text{175B}}$   &(\text{self}\text{-amplified})  & \textbf{30.0}   & \textbf{31.8}    \\ 
    $\text{mT5}_{\text{3.7B}}$\ $+$ \ \text{\textsc{Sap}}  &(\text{self}\text{-amplified})       & 29.8            & 31.4             \\ 
    \bottomrule[\heavyrulewidth]
    \end{tabularx}
    \caption{Unsupervised zero-shot machine translation results on WMT14 English-French test set (SacreBLEU) \citep{wmt14,sacrebleu}. $\text{GPT-3}_{\text{175B}}\ \text{(self-amplified)}$ results correspond to the unsupervised zero-shot ``GPT-3 (self-amplified)'' results from \citet{gpt3unsupervised} prior to performing distillation, initial backtranslation, and iterative backtranslation which involved unsupervised weight updates. $\text{mT5}_{\text{3.7B}}\ \text{(self-amplified)}$ is our fully unsupervised zero-shot approach outlined in Section \ref{sec:zero-shot} with a 16 prompt ensemble. The SacreBLEU signature used also follows \citet{gpt3unsupervised}: \\{\small\texttt{BLEU+case.mixed+numrefs.1+smooth.exp+tok.intl+version.1.2.20})}}
    \label{table:selfamplification}
    \end{table}
}
